Push-Pull: Characterizing the Adversarial Robustness for Audio-Visual Active Speaker Detection

Audio-visual active speaker detection (AVASD) is well-developed, and now is an indispensable front-end for several multi-modal applications. However, to the best of our knowledge, the adversarial robustness of AVASD models hasn't been investigated, not to mention the effective defense against such attacks. In this paper, we are the first to reveal the vulnerability of AVASD models under audio-only, visual-only, and audio-visual adversarial attacks through extensive experiments. What's more, we also propose a novel audio-visual interaction loss (AVIL) for making attackers difficult to find feasible adversarial examples under an allocated attack budget. The loss aims at pushing the inter-class embeddings to be dispersed, namely non-speech and speech clusters, sufficiently disentangled, and pulling the intra-class embeddings as close as possible to keep them compact. Experimental results show the AVIL outperforms the adversarial training by 33.14 mAP (%) under multi-modal attacks.

==> figure_and_table/exp_table_comparison.tex <==
% Ablation Study of the embedding loss of AVADL new
\begin{table}[ht]
% \vspace*{-0.5cm}
\renewcommand{\tabcolsep}{4.5pt}
\renewcommand\arraystretch{0.9}
\fontsize{8}{10}\selectfont
% \fontsize{9}{9}\selectfont
\centerline{
\begin{tabular}{c|c|c|c|c}
\hline
\multirow{2}{*}{\shortstack[c]{Model ($\mathcal{L}_{{CE}_{all}}$)}} & Clean & BIM & MIM & PGD \\
\cline{2-5}
&   mAP (\%) &  mAP (\%) &  mAP (\%)&  mAP (\%) \\

\hline
(A)    & 92.58   &   49.53    &   49.30  & 47.79 \\
(B1)   & 92.15   &   62.70    &   59.26  & 60.01 \\
(B2)   & 91.34   &   54.66    &   52.18  & 54.23 \\
(B3)   & 91.68   &   58.29    &   58.30  & 56.06 \\
(D3)   & 91.81   &   93.86    &   93.34  & 93.15 \\
(E1)   & 90.63   &   97.85    &   97.60  & 97.47 \\
(E2)   & 91.70   &   \textbf{99.99}  &   \textbf{99.98}  & \textbf{99.97} \\
(E3)   & 91.88   &   97.68    &   97.47  & 98.67 \\
\hline
\multirow{2}{*}{\shortstack[c]{Model ($\mathcal{L}_{{CE}_{av}}$)}} & Clean & BIM & MIM & PGD \\
\cline{2-5}
&   mAP (\%) &  mAP (\%) &  mAP (\%)&  mAP (\%) \\
\hline
(A$'$)    & 92.58   &  56.47  & 54.11 &  54.81  \\
(B1$'$)   & 92.15   &  67.48  & 65.26 &  64.59  \\
(B2$'$)   & 91.34   &  65.23  & 67.92 &  59.84  \\
(B3$'$)   & 91.68   &  68.09  & 65.63 &  66.09  \\
(D3$'$)   & 91.81   &  97.25  & 96.83 &  98.37  \\
(E1$'$)   & 90.63   &  98.36  & 98.06 &  97.63  \\
(E2$'$)   & 91.70   &  \textbf{99.97}  & \textbf{99.99} &  \textbf{99.99}  \\
(E3$'$)   & 91.88   &  98.43  & 98.60 &  96.81  \\
\hline
\end{tabular}}
% \vspace*{-0.3cm}
\caption{Training-aware vs inference-aware attack scenarios.}
\label{tab:diiferent_scenerio}
\end{table}



==> figure_and_table/exp_table_multi-attack.tex <==
\begin{table*}[ht!]
    \setlength{\tabcolsep}{1.0pt}
    \renewcommand\arraystretch{1.3}
    % \fontsize{8}{12}\selectfont
   \fontsize{8}{10}\selectfont
    \center
    \begin{tabular}{lc|c|ccc|ccc|ccc|ccc|ccc} 
\hline
    &\multirow{3}{*}{\shortstack[c]{Model}} & \multirow{3}{*}{\shortstack[c]{Attack \\ Method}} &    \multicolumn{15}{c}{ mAP (\%) of different attack strength $\epsilon$ under different attack modalities}    \\
\cline{4-18}
&&& \multicolumn{3}{c|}{$\epsilon_a=0.0001$, $\epsilon_v=0.1$} & \multicolumn{3}{c|}{$\epsilon_a=0.0002$, $\epsilon_v=0.2$} & \multicolumn{3}{c|}{$\epsilon_a=0.0003$, $\epsilon_v=0.3$} & \multicolumn{3}{c|}{$\epsilon_a=0.0004$, $\epsilon_v=0.4$} & \multicolumn{3}{c}{$\epsilon_a=0.0005$, $\epsilon_v=0.5$} \\ 

\cline{4-18}
     & &  & Audio & Visual & Both & Audio & Visual & Both & Audio & Visual & Both & Audio & Visual & Both & Audio & Visual & Both \\

\hline

                                    %% Audio    Visual    Both  %%
               (a) & Baseline    & None &  100   &  100   &    100    \ 
                                 &  100   &  100   &    100    \ 
                                 &  100   &  100   &    100    \ 
                                 &  100   &  100   &    100    \ 
                                 &  100   &  100   &    100    \\
\hline
                                    %% Audio    Visual    Both  %%
(b) & ncTalkNet-TalkNet  & \multirow{3}{*}{BIM}  & 99.99 & 98.89 & 98.90 \
                                           & 99.99 & 98.77 & 98.81 \
                                           & 99.98 & 98.80 & 98.68 \
                                           & 99.98 & 98.85 & 98.90 \
                                           & 99.97 & 98.88 & 98.71 \\

                                     %% Audio    Visual    Both  %%
(c) & specTalkNet-TalkNet   &              & 99.99 & 99.45 & 99.49 \
                                           & 99.97 & 99.43 & 99.35 \
                                           & 99.97 & 99.47 & 99.48 \
                                           & 99.96 & 99.58 & 99.45 \
                                           & 99.96 & 99.47 & 99.45 \\
                                 
                                      %% Audio    Visual    Both  %%
(d) & TalkNet-TalkNet  & & 99.97 & 85.24 & 82.81 \
                         & 99.82 & 81.40 & 75.84 \
                         & 99.65 & 78.66 & 70.66 \
                         & 99.35 & 76.94 & 67.48 \
                         & 99.14 & 77.34 & \textbf{65.45} \\
\hline
                                    %% Audio    Visual    Both  %%
(e) & ncTalkNet-TalkNet & \multirow{3}{*}{MIM}  &  99.99  &  98.91  &  98.93  \
                                           &  99.99  &  98.8   & 98.85  \
                                           &  99.99  &  98.78  & 98.81  \
                                           &  99.98  &  98.85  & 98.97 \
                                           & 99.98   &  98.88  & 98.88 \\

                                     %% Audio    Visual    Both  %%
(f) & specTalkNet-TalkNet &                & 99.99  &  99.54  &  99.53 \
                                           & 99.97  &  99.38  &  99.39 \
                                           & 99.96  &  99.46  &  99.45 \
                                           & 99.97  &  99.54  &  99.53  \
                                           & 99.95  &  99.54  &  99.37  \\
                                 
                                      %% Audio    Visual    Both  %%
(g) & TalkNet-TalkNet  & &  99.97  & 85.30  & 82.86  \
                         &  99.85  & 81.24  & 75.67  \
                         &  99.61  & 78.58  & 70.77  \
                         &  99.42  & 77.17  & 67.45  \
                         &  99.15  & 77.65  & \textbf{65.23}  \\
\hline

                                    %% Audio    Visual    Both  %%
(h) & ncTalkNet-TalkNet  & \multirow{3}{*}{PGD} & 99.99 & 98.89 & 98.88 \
                                          & 99.99 & 98.82 & 98.69 \
                                          & 99.98 & 98.85 & 98.85 \
                                          & 99.98 & 98.82 & 98.87 \
                                          & 99.97 & 98.89 & 98.77 \\

                                     %% Audio    Visual    Both  %%
(i) & specTalkNet-TalkNet &                      & 99.99 & 99.50 & 99.50 \
                                          & 99.97 & 99.44 & 99.38 \
                                          & 99.96 & 99.50 & 99.45 \
                                          & 99.96 & 99.51 & 99.41 \
                                          & 99.95 & 99.58 & 99.47 \\
                                 
                                      %% Audio    Visual    Both  %%
(j) & TalkNet-TalkNet  && 99.97 & 85.27 & 83.0  \
                        & 99.85 & 81.18 & 75.7  \
                        & 99.66 & 78.72 & 70.45 \
                        & 99.38 & 77.15 & 66.94 \
                        & 99.04 & 77.04 & \textbf{65.20} \\
\hline
\vspace{-0.5em}
\end{tabular}
\caption{Adversarial attack performance on AVASD models under audio-only, visual-only and bi-modal attacks by different attack algorithms in black-box scenarios (b), (c), (e), (f), (h), (i); and white-box scenarios (d), (g) and (j). }
\label{tab:adv_attack_AVASD}
\vspace{-1em}
\end{table*}

